Relaxation Deferred Correction Methods and their Applications to Residual Distribution Schemes

In [1] is proposed a simplified DeC method, that, when combined with the residual distribution (RD) framework, allows to construct a high order, explicit FE scheme with continuous approximation avoiding the inversion of the mass matrix for hyperbolic problems. In this paper, we close some open gaps in the context of deferred correction (DeC) and their application within the RD framework. First, we demonstrate the connection between the DeC schemes and the RK methods. With this knowledge, DeC can be rewritten as a convex combination of explicit Euler steps, showing the connection to the strong stability preserving (SSP) framework. Then, we can apply the relaxation approach introduced in [2] and construct entropy conservative/dissipative DeC (RDeC) methods, using the entropy correction function proposed in [3]. [1] R. Abgrall. High order schemes for hyperbolic problems using globally continuous approximation and avoiding mass matrices. Journal of Scientific Computing, 73(2):461--494, Dec 2017. [2] D. Ketcheson. Relaxation Runge--Kutta methods: Conservation and stability for inner-product norms. SIAM Journal on Numerical Analysis, 57(6):2850--2870, 2019. [3] R. Abgrall. A general framework to construct schemes satisfying additional conservation relations. application to entropy conservative and entropy dissipative schemes. Journal of Computational Physics, 372:640--666, 2018.

==> numericsODE.tex <==




\subsection{Numerical test in the ODE case}
In this section we validate the ideas presented in \cref{sec:RDeCConservatiteDavide,sec:RDeCDissipativeDavide} for systems of ODEs
\begin{equation}
	\partial_t U +F(U)=0, \quad t\in[0,T],
\end{equation}
where $U(t)\in \R^D$ and $F:\R^D\to\R^D$ is a Lipschitz continuous function. In this context, the residual $\Phi_x$ in \cref{sec:RDeCConservatiteDavide,sec:RDeCDissipativeDavide} become simply the function $F$ and the mass matrix and the diagonal matrix are trivially the identity matrix.

\subsubsection{Nonlinear oscillator}
The first test we consider is a nonlinear oscillator system defined as the initial value problem
\begin{equation}
	\begin{cases}
	\partial_t \begin{pmatrix}
		u_1\\u_2
	\end{pmatrix}= \begin{pmatrix}
	\frac{-u_2}{n} \\\frac{u_1}{n}
\end{pmatrix}, \qquad \text{ with } n:=\sqrt{u_1^2+u_2^2},\\
		u_1(0) = u_1^0,	\\ u_2(0) = u_2^0.
	\end{cases}
\end{equation}

The system verify the exact solution
\begin{equation}
	\begin{pmatrix}
		u_1(t)\\u_2(t)
	\end{pmatrix} = \begin{pmatrix}
	\cos(\theta) & -\sin(\theta)\\
	\sin(\theta) & \cos(\theta)
\end{pmatrix}\begin{pmatrix}
u_1^0\\u_2^0
\end{pmatrix}, \quad \theta(t):=\frac{t}{n}.
\end{equation}
One can verify that the system conserve the energy $n$ in time. \todo{really I guesss at least n^2}
Testing the DeC and the relaxation DeC (RDeC), we observe differences in the energy of the systems.
\begin{figure}
	\begin{subfigure}{1\textwidth}
		\includegraphics[width=0.62\linewidth]{../Plots/ODEs/Pendolum_Simulation_RDeC6_N35.pdf}
	\includegraphics[width=0.37\linewidth]{../Plots/ODEs/Pendolum_Phase_RDeC6_N35.pdf}
	\caption{Simulation for order 6 and $N=35$: time evolution (left), phase space (right)}\label{fig:nonLinOscillatorDeC6}
\end{subfigure}

\begin{subfigure}{1\textwidth}
	\includegraphics[width=0.62\linewidth]{../Plots/ODEs/Pendolum_Simulation_RDeC2_N47.pdf}
	\includegraphics[width=0.37\linewidth]{../Plots/ODEs/Pendolum_Phase_RDeC2_N47.pdf}
	\caption{Simulation for order 2 and $N=47$: time evolution (left), phase space (right)}\label{fig:nonLinOscillatorDeC2}
\end{subfigure}

\begin{subfigure}{1\textwidth}
	\includegraphics[width=0.49\linewidth]{../Plots/ODEs/Pendolum_Energy_comparison.pdf}
	\includegraphics[width=0.49\linewidth]{../Plots/ODEs/Pendulum_gammas_comparison.pdf}
	\caption{Energy (left) and $\gamma$ (right) comparison for RDeC orders 2 and 6 with $N=50$}\label{fig:nonLinOscillatorComparison}
\end{subfigure}
\caption{Simulation of the nonlinear oscillator for DeC and RDeC of orders 2 and 6} \label{fig:nonLinOscillatorSimulations}
\end{figure}
In \cref{fig:nonLinOscillatorSimulations} the simulations for the nonlinear oscillator problems are depicted for DeC and RDeC of order 2 and 6 for different number of timesteps. In the high order solutions in \cref{fig:nonLinOscillatorDeC6} we can not observe qualitatively a difference between DeC and RDeC, but for the second order method in \cref{fig:nonLinOscillatorDeC2} it is evident that the DeC increases the energy of the system violating the physical bounds.

Computing the norm of the energy and its evolution in \cref{fig:nonLinOscillatorComparison} we observe a perfect maintaining of the total energy of the RDeC schemes, while the DeC are going away from the exact values with the respective order of accuracy.

Finally, we observe in \cref{fig:nonLinOscillatorConvergence} that there are several phenomena of super convergence in this test. In particular in the case of equispaced points we fall back in the superconvergence of the odds orders as already shown in \cite{ketcheson2019_RRK_rr}, while for Gauss Lobatto nodes we have even further phenomena of super convergence. Only order 2 is not affected by this.
\begin{figure}
\begin{subfigure}{0.49\textwidth}
   \includegraphics[width=\linewidth]{../Plots/ODEs/Pendolum_convergence_equispaced.pdf}
   \caption{Equispaced subtimesteps}\label{fig:nonLinOscillatorConvergenceEqui}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\linewidth]{../Plots/ODEs/Pendolum_convergence_gaussLobatto.pdf}
\caption{Gauss Lobatto subtimesteps}\label{fig:nonLinOscillatorConvergenceGLB}
\end{subfigure}
\caption{Convergence error of DeC and RDeC methods for nonlinear oscillator}\label{fig:nonLinOscillatorConvergence}
\end{figure}

\subsubsection{Damped nonlinear oscillator}
The second ODE we consider is a damped version of the previous nonlinear oscillator.
It is defined by the initial value problem\begin{equation}
	\begin{cases}
		\partial_t \begin{pmatrix}
			u_1\\u_2
		\end{pmatrix}= \begin{pmatrix}
			\frac{-u_2}{n} -\alpha u_1\\\frac{u_1}{n}-\alpha u_2
		\end{pmatrix}, \qquad \text{ with } n:=\sqrt{u_1^2+u_2^2},\\
		u_1(0) = u_1^0,	\\ u_2(0) = u_2^0.
	\end{cases}
\end{equation}
The final time is set to $T=100$.
The system verify the exact solution
\begin{equation}
	\begin{pmatrix}
		u_1(t)\\u_2(t)
	\end{pmatrix} = \begin{pmatrix}
		\cos(\theta) & -\sin(\theta)\\
		\sin(\theta) & \cos(\theta)
	\end{pmatrix}\begin{pmatrix}
		u_1^0\\u_2^0
	\end{pmatrix}, \quad n(t)=n(0) e^{-\alpha t}, \quad \theta(t):=\frac{1}{\alpha n(0)}\left(e^{\alpha t}-1\right).
\end{equation}
This problem is much harder to be solved numerically as the oscillations have frequencies that increase with time and tends to infinity. So, we need to use many more timesteps. 
In \cref{fig:DampnonLinOscillatorDeC6,fig:DampnonLinOscillatorDeC2} we show the simulations and the phase values till time 100 for the RDeC and DeC of order 6 and 2 respectively. As before, qualitatively the high order methods are both precise, while the second order methods show large differences, DeC2 does not catch at all the decrease in time of the energy and hence the increase of frequency, while RDeC2 is much more accurate.

In \cref{fig:DampnonLinOscillatorComparison} we can observe the different errors of the energy from the exact one and clearly the high order methods are much more precise. Morever, we can state that the relaxed DeCs are around one order of magnitude more precise in catching the energy level.
\begin{figure}
	\begin{subfigure}{1\textwidth}
		\includegraphics[width=0.62\linewidth]{../Plots/ODEs/DampPendolum_Simulation_RDeC6_N250.pdf}
		\includegraphics[width=0.37\linewidth]{../Plots/ODEs/DampPendolum_Phase_RDeC6_N250.pdf}
		\caption{Simulation for order 6 and $N=250$: time evolution (left), phase space (right)}\label{fig:DampnonLinOscillatorDeC6}
	\end{subfigure}
	
	\begin{subfigure}{1\textwidth}
		\includegraphics[width=0.62\linewidth]{../Plots/ODEs/DampPendolum_Simulation_RDeC2_N250.pdf}
		\includegraphics[width=0.37\linewidth]{../Plots/ODEs/DampPendolum_Phase_RDeC2_N250.pdf}
		\caption{Simulation for order 2 and $N=250$: time evolution (left), phase space (right)}\label{fig:DampnonLinOscillatorDeC2}
	\end{subfigure}
	
	\begin{subfigure}{1\textwidth}
		\includegraphics[width=0.49\linewidth]{../Plots/ODEs/DampPendolum_Energy_comparison.pdf}
		\includegraphics[width=0.49\linewidth]{../Plots/ODEs/DampPendulum_gammas_comparison.pdf}
		\caption{Energy (left) and $\gamma$ (right) comparison for RDeC orders 2 and 6 with $N=50$}\label{fig:DampnonLinOscillatorComparison}
	\end{subfigure}
	\caption{Simulation of the damped nonlinear oscillator for DeC and RDeC of orders 2 and 6} \label{fig:DampnonLinOscillatorSimulations}
\end{figure}
In \cref{fig:DampnonLinOscillatorConvergence} we observe similar superconvergence results as in the previous test.
\begin{figure}
	\begin{subfigure}{0.49\textwidth}
		\includegraphics[width=\linewidth]{../Plots/ODEs/DampPendolum_convergence_equispaced.pdf}
		\caption{Equispaced subtimesteps}\label{fig:DampnonLinOscillatorConvergenceEqui}
	\end{subfigure}
	\begin{subfigure}{0.49\textwidth}
		\includegraphics[width=\linewidth]{../Plots/ODEs/DampPendolum_convergence_gaussLobatto.pdf}
		\caption{Gauss Lobatto subtimesteps}\label{fig:DampnonLinOscillatorConvergenceGLB}
	\end{subfigure}
	\caption{Convergence error of DeC and RDeC methods for nonlinear oscillator}\label{fig:DampnonLinOscillatorConvergence}
\end{figure}
